Collectively Simplifying Trajectories in a Database: A Query Accuracy Driven Approach

Increasing and massive volumes of trajectory data are being accumulated that may serve a variety of applications, such as mining popular routes or identifying ridesharing candidates. As storing and querying massive trajectory data is costly, trajectory simplification techniques have been introduced that intuitively aim to reduce the sizes of trajectories, thus reducing storage and speeding up querying, while preserving as much information as possible. Existing techniques rely mainly on hand-crafted error measures when deciding which point to drop when simplifying a trajectory. While the hope may be that such simplification affects the subsequent usability of the data only minimally, the usability of the simplified data remains largely unexplored. Instead of using error measures that indirectly may to some extent yield simplified trajectories with high usability, we adopt a direct approach to simplification and present the first study of query accuracy driven trajectory simplification, where the direct objective is to achieve a simplified trajectory database that preserves the query accuracy of the original database as much as possible. Specifically, we propose a multi-agent reinforcement learning based solution with two agents working cooperatively to collectively simplify trajectories in a database while optimizing query usability. Extensive experiments on four real-world trajectory datasets show that the solution is capable of consistently outperforming baseline solutions over various query types and dynamics.

==> introduction-bak.tex <==
\section{INTRODUCTION}
\label{sec:intro}

Massive amounts of trajectory data are being accumulated and used in diverse applications, such as discovering popular routes in a city~\cite{chen2011discovering}, analyzing animal migration patterns~\cite{li2011movemine}, and perform sports analytics~\cite{wang2019effective}. A trajectory is a sequence of time-stamped locations that describe the movement of an object over time.

The accumulation of trajectory data~\cite{wang2021error} introduces at least two challenges
%, which have been demonstrated in many recent trajectory survey
~\cite{lin2021error,zhang2018trajectory}: (1) storing the data is expensive, and (2) querying the data is time-consuming. These challenges can be addressed by conducting trajectory simplification, which aims to drop points from trajectories to save the storage cost and speed up query processing. 
%Correspondingly, the query efficiency is improved. 
The underlying rationale is that not all points in a trajectory carry equally important information, so that dropping unimportant ones may be acceptable. For example, if the location of an object is sampled regularly and the object does not move for a while then only the first and last positions during the period of inactivity are important, and those in-between may be dropped without loosing information.
%affect the results apparently. 
Next, the efficiency of query processing is improved, at the expense of query results becoming approximate.
% although the query results may not be accurate.
%, since the trajectory that is stored becomes shorter.

Indeed, the extent to which a collection of simplified trajectories enables accurate query results has been used widely as a measure of the quality of a simplification technique in empirical studies of trajectory simplification~\cite{cao2006spatio,lin2021error,zhang2018trajectory}. 
For example, Zhang et al.~\cite{zhang2018trajectory} evaluate existing simplification techniques in terms of their ability to produce simplified trajectories that affect the accuracy of range, $k$NN, and join queries as well as clustering minimally. 
%
% However, none of the previous trajectory simplification algorithms~
While there are many proposals for trajectory simplification~\cite{hershberger1992speeding,keogh2001online,long2014trajectory,wang2021trajectory,potamias2006sampling,muckell2011squish,muckell2014compression}, they all assume a storage budget and aim to produce simplified trajectories that minimize the difference from the original trajectories according to a given difference notion.
No proposals aim to optimize directly the query accuracy offered by the simplified trajectories.
% as their optimization objective directly. % Instead, they
%
We call this line of study \emph{Error-Driven Trajectory Simplification (EDTS)}. 
% For example, the Top-Down~\cite{hershberger1992speeding} algorithm first includes the first and last points into a simplified trajectory, and then it defines a heuristic error (e.g., synchronous Euclidean distance (SED)) on each point to be included, and it repetitively includes the point with the largest error into a simplified trajectory until the number of points reaches the given budget. 

%Bottom-Up is a reversed version of Top-Down, where it repeatedly drops the point with the smallest error~\cite{keogh2001online} in a trajectory. 

%RLTS+~\cite{wang2021error} adopts the strategy of Bottom-Up, and achieves a more intelligent method to drop points with reinforcement learning. 

%Overall, how to preserve query accuracy is not their focus, and cannot be explicitly optimized with those errors.

In addition, existing simplification techniques are local in nature and operate on a per-trajectory basis as opposed to being global in nature and operating on a database of trajectories. Specifically, they aim to simplify a given trajectory $T$ within a budget $r\cdot |T|$, where $r$ is the compression ratio. When these techniques are used to simplify a database of trajectories according to a compression ratio $r$, they simplify each trajectory in the database \emph{separately} according to compression ratio $r$. This is likely sub-optimal in cases where trajectories have different sampling rates or different complexities. Intuitively, trajectories with higher sampling rates or lower complexity are candidates for simplification with larger compression ratios.

Therefore, we propose a new trajectory simplification problem, called \emph{Query accuracy Driven Trajectory Simplification (QDTS)}. Given a trajectory database $D$ and a storage budget, the problem is to find a simplified trajectory database $D'$ that preserves the accuracy of query results as much as possible, compared to the query results on $D$. 
% To our best knowledge, the QDTS problem is the first systematic study on this line of trajectory simplification. 
QDTS differs from the existing EDTS problem. First, it considers a different objective of trajectory simplification, namely that of preserving query accuracy directly, rather than through minimizing an error measure, as in the EDTS problem. Second, it is global in nature and takes a trajectory database as input and outputs a simplified trajectory database that satisfies a specified storage budget as a whole, instead of simplifying each trajectory in isolation according to a budget, as do existing EDTS techniques~\cite{hershberger1992speeding,keogh2001online,wang2021error}.

%To answer the QDTS problem, 
%a core problem is to preserve the trajectories they would be queried out from the simplified database. However, it is hard to infer the potential queries on a database. Here, 
% we propose a 
% %data-driven 
% reinforcement learning based solution. 
% We model the query-driven trajectory simplification process as a Markov decision process (MDP), whose objective (i.e., preserving the query accuracy) is explicitly optimized with reinforcement learning. 
We develop a solution to the QDTS problem that is based on reinforcement learning.
It starts with the most simplified database, in which each simplified trajectory $T'$ of an original trajectory $T$ consists of only the first and last points of $T$. It then introduces original points into the simplified database iteratively until the budget is exhausted.
%our solution starts with including the first and the last point of each trajectory in a database followed by the trajectory simplification definition. Then, we consider inserting another point among those in the database, such that the point may be severed for queries as much as possible. 
% to achieve the objective, we explore a block sampling based solution. 
This solution differs from existing solutions in two ways.
%
(1) It considers all trajectories in the database \emph{collectively} rather than \emph{separately} as do all existing algorithms. In addition, it partitions the database into spatio-temporal cubes. Then, each time it needs to select a point to introduce, it first identifies a few cubes and considers only points in these cubes as candidates. This improves efficiency.
%do and partitions the database into cubes (among the two spatial dimensions and the temporal dimension). In addition, whenever it needs to select a point, it selects a few cubes first and then focuses the points within the cubes as the candidates of the point to be selected (for better efficiency).
%
(2) It leverages reinforcement learning to learn a policy, instead of using heuristics as do most of the existing algorithms, for selecting points to introduce. The learned policies are query accuracy aware such that they select points that optimize query accuracy.
% We evenly partition a database into cubes. To select a point for simplified database, we randomly sample some cubes, and one point is selected from the points in the sampled cubes. Here, we consider two ways for the sampling. First, 
%we denote the number of trajectories in each block as the data distribution, we consider
% sample a block followed by the data distribution. The rationale behind the sampling is to preserve the distribution on the original database. Second, we uniformly sample a block among all blocks, which aims to take all possible areas of a database into account. 
%We incorporate the sampled blocks where a point is selected within them. 
% To choose a point from the selected blocks, we design a reinforcement learning based solution, where a point is chosen based on the learned policy. The RL based solution provides a more intelligent strategy to choose a point due to its 
%data-driven nature,
% query-driven nature, rather than using some heuristic errors adopted by existing algorithms~\cite{hershberger1992speeding,keogh2001online}.
We call the resulting solution \texttt{RL4QDTS}.

In summary, we make the following contributions. 
\begin{itemize}
    \item We propose the QDTS problem, that aims to find a simplified trajectory database within a given storage budget that preserves query accuracy as much as possible. This is  the first systematic study of this line of trajectory simplification.
    %, it relies on a query processing operator, and we propose a general framework, which could be instantiated   with multiple query processing operators into the framework.
    \item We develop an RL based solution called \texttt{RL4QDTS} to the problem.
    %, which corresponds to the first of its kind. 
    We %formally 
    show that the objective of the QDTS problem can be optimized explicitly by \texttt{RL4QDTS}, and provide theoretical arguments.
    %to verify the soundness of our solution. 
    %Compared with the existing EDTS algorithms, whose objective of trajectory simplification cannot serves various types of queries.
    \item We conduct experiments on two real-world trajectory datasets that offer evidence that \texttt{RL4QDTS} is able to outperform existing EDTS solutions with \emph{two} types of adaptions, \emph{four} error measures, and \emph{varying} storage budgets for \emph{five} query operators.
    %on \emph{both} datasets. 
    % On the other hand, this is also the first work to systematically evaluate the performance of existing trajectory simplification algorithms designed for a single trajectory when being used to simply a trajectory database. 
    %this line of trajectory simplification with respect to those dynamics.
\end{itemize}

The rest of paper is organized as follows. We review the literature in Section~\ref{sec:related}. We cover preliminaries and define the QDTS problem in Section~\ref{sec:problem}.
%
We introduce the \texttt{RL4QDTS} solution in Section~\ref{sec:method}, and we report on the experimental study in Section~\ref{sec:experiment}. We conclude in Section~\ref{sec:con}.

